Provable Defense against Privacy Leakage in Federated Learning from Representation Perspective

Federated learning (FL) is a popular distributed learning framework that can reduce privacy risks by not explicitly sharing private data. However, recent works demonstrated that sharing model updates makes FL vulnerable to inference attacks. In this work, we show our key observation that the data representation leakage from gradients is the essential cause of privacy leakage in FL. We also provide an analysis of this observation to explain how the data presentation is leaked. Based on this observation, we propose a defense against model inversion attack in FL. The key idea of our defense is learning to perturb data representation such that the quality of the reconstructed data is severely degraded, while FL performance is maintained. In addition, we derive certified robustness guarantee to FL and convergence guarantee to FedAvg, after applying our defense. To evaluate our defense, we conduct experiments on MNIST and CIFAR10 for defending against the DLG attack and GS attack. Without sacrificing accuracy, the results demonstrate that our proposed defense can increase the mean squared error between the reconstructed data and the raw data by as much as more than 160X for both DLG attack and GS attack, compared with baseline defense methods. The privacy of the FL system is significantly improved.

==> Intoduction_bak.tex <==
\section{Introduction_bak}\label{sec:Introduction_bak}
Federated learning (FL)~\cite{mcmahan2017communication} is a popular distributed learning framework. In a FL system, remote devices learn local models with their own training data parallely and communicate only local model updates with a central server, where the aggregation will be executed. This scheme allows to train a model using decentralized data  without directly sharing them, and hence overcomes the data privacy issue. 
Therefore, FL has been widely applied to applications where data is distributed across remote devices and contains private information, such as next-word prediction~\cite{hard2018federated}, emoji prediction~\cite{ramaswamy2019federated}, etc.
However, the data is often non-IID (identically and independently distributed) across a massive number of devices in practice. For example, the input words to a virtual keyboard~\cite{hard2018federated} on a mobile phone are often user and context dependent, hence, these text data is highly heterogeneous across devices. 

%Another huge contribution FL brings is that it achieves good performance under data non-iid settings, which is common in real life. FL is widely used in practical applications where data on remote clients contains private information and reveals personalized distributions, such as next-word-prediction on smarts phones and training a model using patients’ medical data from different hospitals.

Distributed learning has been believed to be safe in privacy because private data is not shared in training process. However, recent works have demonstrated that sharing model updates or gradients also makes distributed learning vulnerable to inference attack, e.g., \textit{property inference attack}~\cite{melis2019exploiting} that infers sensitive properties of training data  using the model updates and \textit{reconstruction attack} that recovers training data~\cite{fredrikson2015model, salem2020updates, zhu2019deep, geiping2020inverting, wang2019beyond} using model gradients. However, these works only apply to very simple distributed learning scenarios where a training batch only contains one or a few samples, or there are only a small number of participating devices. FL seems robust to these privacy attacks for its hard and practical setting (large batch size, extensive paticipating devices, e.g.), but we show that it is also vulnerable to privacy problem due to its non-iid characteristics. We will provide an explicit illustration about how communicating model updates only in FL breaches privacy.

In this work, we investigate the key question: \textbf{what privacy information can be inferred about a participating device's training data from the model updates during FL training under non-IID settings?}
We assume the server in FL is malicious, aiming to infer privacy information of training data from participating devices, and the data distribution across devices is non-IID.
We demonstrate the privacy leakage from model updates: the malicious server can perform reconstruction attack and property inference attack using the shared model updates.
demonstrate that communicating model updates leaks training data privacy in FL with the assumption of a malicious server. We analyse and find this leakage flowing from two natures of FL: non-iid data distributions and server's access to local model updates with small training extent. We propose an algorithm that the server can identify data classes each client owns and can even extract the training data representations explicitly for each class of one client's training data from different layers in the uploaded model with very little computational cost only using this client's uploaded models. Our algorithm extracts clients' training data representations in the DNN model in a back-propagation fashion. After extracting the representations in the last layer, we can extract the data representations in previous layers layer by layer. Empirical results demonstrate that the representations our algorithm extracts from the model updates communicated in FL shows as high as 0.99 correlation with the real training data representations extracted by the local model. We also study the influence of the FL training sets on the feature extraction quality, and find that the feature extracted preserve high correlation with the real training data representations even under extremely hard FL training sets.

Having access to the local model and the corresponding data representations from that model, the malicious server can execute inference attack very easily and efficiently. We conduct property inference and model inversion based on the extracted data representations and the uploaded models, and achieve good attack performance. It is notable that with the help of data representations from different layers in the model, the attacks would be extremely efficient. Our feature extraction algorithm does not need any prior about the model convergence, which means that the attack does not depend on training status in FL. To prevent data feature leakage in FL, we demonstrate x defense strategies: xxxxx 

 Our key contributions can be summarized as follows:
 \begin{itemize}
    \item We demonstrate communicating model parameters leaks data privacy in FL and provide an explicit illustration about the essential cause of this leakage.
    \item We propose an algorithm that can identify each client's data classes and extract each client's training data representations using transmitted local models with very little computation cost. To our best acknowledgement, this is the first algorithm achieving it.
    \item Based on the training data feature extraction algorithm, we conduct several privacy attacks on FL and provide the empirical attack results. We also provide several defense strategies against this training feature leakage.
\end{itemize}

==> attack.tex <==
\section{Privacy leakage attack}

\subsection{Threat model}
\subsection{Model inversion}
\subsection{Property inference}

==> experiments_bak.tex <==
\section{Experiments}\label{sec:experiments_bak}

\subsection{Representation extraction}
\paragraph{setup}
To mimic realistic settings, we choose CIFAR10 \cite{krizhevsky2009learning} and MNIST \cite{lecun1995learning} datasets and follow the \textbf{2-class \& balanced} configuration in \cite{li2020lotteryfl} to construct non-IID datasets. There are totally 100 devices and 10 devices are involved in training during each communication round. Each device owns 2 class of data and we specify the number of samples per class on a device as 20. 

As analysed in Section \ref{sec:cause1}, representation extraction is effected by the local training settings. We vary local epoch $E \in \{ 1, 5, 10\}$ and local batch size $B \in \{ 8, 16, 32\}$. We use SGD \cite{} as the optimizer with learning rate $\eta$ 0.01 and set $M$ in Algorithm \ref{alg:extraction} as 1. The base model architectures corresponding to CIFAR10 and MNIST can be found in Appendix.

To illustrate that the non-IID characteristic of FL is one major cause of representation leakage, we also centralize the data on one device to mimic centralized training. For this setting, $E$ is set to be 1 and $B$ is 32.


\paragraph{evaluation metric}

As shown in Section \ref{sec:method}, the data representation $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ we extract approximates the linear scaled data representation $\overline{\va}_{\sB_i}^{\mathrm{T}}$, where the scale $\gamma$ is related to the local training settings. Thus, we apply correlation coefficient \cite{benesty2009pearson} $r$ to evaluate the linear similarity between the extracted representation $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ and the real data representation $\overline{\va}_{\sB_i}^{\mathrm{T}}$. We compute $r$ between $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ and $\overline{\va}_{\sB_i}^{\mathrm{T}}$ for each data class on each device participating in this communication round. We report the average $r$ across data classes and devices as the $r$ in this communication round.

\paragraph{results}

We extract data representations from all fully connected layers in all 200 communication rounds, and the average $r$ across all communication rounds is reported in Table \ref{tb:r_average}.

\begin{table}[t]
    \centering
    \caption{average $r$ across 200 communication rounds for different layers under different settings.}
        \begin{tabular}{l || c c |c c c}
            \toprule
            \multirow{2}*{Local training settings} & \multicolumn{2}{c|}{MNIST} & \multicolumn{3}{c}{CIFAR10} \\
            \cline{2-6}
            \multirow{2}*{} & FC1 & FC2 & FC1 & FC2 & FC3 \\
            \hline
            E=1, B=32 & 0.88 & 0.91 & 0.98 & 0.99 & 0.99 \\
            \hline
            E=5, B=32 & 0.50 & 0.80 & 0.82 & 0.90 & 0.92 \\
            \hline
            E=10, B=32 & 0.39 & 0.78 & 0.70 & 0.78 & 0.82 \\
            \hline
            E=1, B=16 & 0.60 & 0.83 & 0.82 & 0.93 & 0.99 \\
            \hline
            E=1, B=8 & 0.38 & 0.74 & 0.85 & 0.89 & 0.92 \\
            \hline
            E=1, B=32 (Centralized) & 0.11 & 0.09 & 0.48 & 0.31 & 0.18 \\
            \bottomrule
            
        \end{tabular}
    \label{tb:r_average}
\end{table}

It is shown that the the data representations we extracted $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ has as high as 0.99 correlation with the real training data representations $\overline{\va}_{\sB_i}^{\mathrm{T}}$, which proves the serious representation leakage in FL. When local training step ($K$ in Equation \ref{eq:fc_grad_MB_approx}) increases (higher E, lower B), the average correlation decreases, which is reasonable according to the discussion in Section \ref{sec:cause1}. However, $r$ is still higher than 0.8 for some layers even under the setting where $E$ is 10 and it is notable that the local training step ($K$) should not be too high \cite{mcmahan2017communication} if you want to achieve good performance in FL. $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ and $\overline{\va}_{\sB_i}^{\mathrm{T}}$ have super low correlation coefficient under the centralized setting, which proves that the non-IID characteristic is a major cause of representation leakage.

Under the same local training setting, the correlation between $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ and $\overline{\va}_{\sB_i}^{\mathrm{T}}$ is lower in shallower layers (layers closer to the input layer). This is because the data representations in the shallower layers are more general[], thus the structural specification of $Grad_{\sB}(i)$ in Equation \ref{eq:fc_grad_B} according to different data classes will be lower. As a result, the representation extraction in shallower layers will be harder compared to deeper layers.

\begin{figure}[h]
    \centering
    \subfigure[FC1]{
    \centering
    \includegraphics[scale=\scale]{images/cifar10_fc1.eps}}
    \subfigure[FC2]{
    \centering
    \includegraphics[scale=\scale]{images/cifar10_fc2.eps}}
    \subfigure[FC3]{
    \centering
    \includegraphics[scale=\scale]{images/cifar10_fc3.eps}
    }
    \caption{$r$ in different layers during communication rounds for CIFAR10}
    
    \label{fig:cifar10_fc}
\end{figure}{}

To study the relationship between $r$ and training process, we document average $r$ in each communication round and visualize it in Figure \ref{fig:cifar10_fc}. It is shown that $r$ drops along with the communication rounds. This kind of drop comes from the lower updates of local parameters when training process is going on. Lower updates means less data representations embedded in model updates, which makes the extraction harder. However, $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ still has more than 75\% correlation with $\overline{\va}_{\sB_i}^{\mathrm{T}}$ in the last layer and becomes stable in the later communication rounds.




\subsection{Inference attack}
Having access to the model and the data representations, the malicious server can conduct different types of privacy inference attacks. We conduct model inversion and property inference here to demonstrate the danger of representation leakage in FL.

\paragraph{Threat model} 
Following the training process of FL described in \cite{mcmahan2017communication}, we assume that $D (D\ge2)$ devices participate in federated training. For one device, its data show strong personalization and involve privacy information. We assume a malicious server aiming at reconstructing a data point showing the training data privacy information or inferring private properties in training data for each class on one device. The server has only access to the model parameters the devices uploaded and analyses the privacy information through the model parameters and the parameter updates.

\paragraph{setup}

We consider facial recognition scenario and use ORL database of Cambridge to conduct inference attacks. We set up 40 devices and each device is distributed the facial images of one person. By doing this, we mimic the real world that users want to train models recognize their own faces. In each communication round, 10 devices are involved in training. We set local epoch $E$ to be 10 and batch size $B$ to be 32. The base model architecture can be found in Appendix. 

\paragraph{Model inversion}


\begin{figure}[h]
\centering
     \includegraphics[scale=0.4]{images/inversion.png}
\caption{Model inversion results. The right first }
\label{fig:inversion}
\end{figure}

After the malicious server identifies the training class $i$ for one device and extracts the corresponding data representation $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}} \in \sR^{Q}$ in one layer of this device's model following Algorithm \ref{alg:extraction}, it can perform model inversion attack with $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}$ and the local model parameters. The server reconstruct the data point $x_i\in \sR^{P}$ by minimizing the following objective

\begin{equation}
x_i = \mathop{\arg\max}_{x_i} corr(\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}}, \Phi (x_i))
\label{eq:inversion}
\end{equation}

where $corr(a, b)$ denotes correlation coefficient between $a$ and $b$. $\Phi: \sR^{P} \rightarrow \sR^{Q}$ is the representation function in the uploaded local model that generate the data representation $\overline{\va}_{\sB_i}^{\mathrm{T}}$ in the corresponding layer. The server conducts attack after 50 communication rounds. We visualize the earliest inversion results for some devices in Figure \ref{fig:inversion}. It can be shown that the reconstructing results are better when using shallower representations, which illustrates the danger of representation leakage in multiple layers.

\paragraph{Property inference}

After extracting one layer's data representation $\hat{\overline{\va}}_{\sB_i}^{\mathrm{T}} \in \sR^{q}$ from one device, the malicious server can infer the private properties of the training data in $\sB_i$ of this device with some public labeled data points. For a private property, we assume the server has some labeled data points $\{X' \in \sR^{K \times P}, Y' \in \sR^{K \times 1}\}$ and compute the data representations $\{R' \in \sR^{K \times Q}\}$ of $\{X'\}$ with the representation function $\Phi: \sR^{P} \rightarrow \sR^{Q}$ in the uploaded local model from one device. Then the server can train a property classifier $f: \sR^{Q} \rightarrow \sR$ for this device using $\{R', Y'\}$.

We choose the properties of {\bf{gender}} and {\bf{wearing glass}} as the inference targets and infer these two properties of the facial data on each device. The average inference accuracies are listed in Table{}. The detailed experiment settings can be found in Appendix. 

==> input.tex <==
\input input

